Robust Lane Detection with Wavelet-Enhanced Context Modeling and Adaptive Sampling

Lane detection is critical for autonomous driving and ad-vanced driver assistance systems (ADAS). While recent methods like CLRNet achieve strong performance, they struggle under adverse con-ditions such as extreme weather, illumination changes, occlusions, and complex curves. We propose a Wavelet-Enhanced Feature Pyramid Net-work (WE-FPN) to address these challenges. A wavelet-based non-local block is integrated before the feature pyramid to improve global context modeling, especially for occluded and curved lanes. Additionally, we de-sign an adaptive preprocessing module to enhance lane visibility under poor lighting. An attention-guided sampling strategy further reffnes spa-tial features, boosting accuracy on distant and curved lanes. Experiments on CULane and TuSimple demonstrate that our approach signiffcantly outperforms baselines in challenging scenarios, achieving better robust-ness and accuracy in real-world driving conditions.

==> tables/culane.tex <==
\begin{table*}

    \begin{center}

        \resizebox{\textwidth}{!}{%

            \begin{tabular}{@{}lrrrrrrrrrrrrrrr@{}}

                \toprule

                \multicolumn{1}{c}{\textbf{Method}} & \multicolumn{1}{c}{\textbf{Backbone}} & \multicolumn{1}{c}{\textbf{mF1}} &
                \multicolumn{1}{c}{\textbf{F1@50}} &
                \multicolumn{1}{c}{\textbf{F1@75}} &
                \multicolumn{1}{c}{\textbf{Normal}} & \multicolumn{1}{c}{\textbf{Crowded}} & \multicolumn{1}{c}{\textbf{Dazzle}} & \multicolumn{1}{c}{\textbf{Shadow}} & \multicolumn{1}{c}{\textbf{No line}} & \multicolumn{1}{c}{\textbf{Arrow}} & \multicolumn{1}{c}{\textbf{Curve}} & \multicolumn{1}{c}{\textbf{Cross}} & \multicolumn{1}{c}{\textbf{Night}} \\ \midrule

                SCNN~\cite{pan2018spatial} & VGG16 & 38.84 & 71.60 & 39.84 & 90.60 & 69.70 & 58.50 & 66.90 & 43.40 & 84.10 & 64.40 & 1990 & 66.10 \\
                
                RESA~\cite{zheng2021resa} & ResNet34 & - & 74.50 & - & 91.90 & 72.40 & 66.50 & 72.00 & 46.30 & 88.10 & 68.60 & 1896 & 69.80  \\

                RESA~\cite{zheng2021resa} & ResNet50 & 47.86 & 75.30 & 53.39 & 92.10 & 73.10 & 69.20 & 72.80 & 47.70 & 88.30 & 70.30 & 1503 & 69.90  \\

                FastDraw~\cite{philion2019fastdraw} & ResNet50 & - & - & -& 85.90 & 63.60 & 57.00 & 69.90 & 40.60 & 79.40 & 65.20 & 7013 & 57.80  \\

                E2E~\cite{yoo2020end} & ERFNet & - & 74.00 & - 91.00 & 73.10 & 64.50 & 74.10 & 46.60 & 85.80 & 71.90 & 2022 & 67.90 \\
                
                UFLD~\cite{qin2020ultra} & ResNet18 & 38.94 & 68.40 & 40.01  & 87.70 & 66.00 & 58.40 & 62.80 & 40.20 & 81.00 & 57.90 & 1743 & 62.10 \\

                UFLD~\cite{qin2020ultra} & ResNet34 & - & 72.30 & - & 90.70 & 70.20 & 59.50 & 69.30 & 44.40 & 85.70 & 69.50 & 2037 & 66.70 \\
                
                PINet~\cite{ko2021key} & Hourglass & 46.81 & 74.40 & 51.33  & 90.30 & 72.30 & 66.30 & 68.40 & 49.80 & 83.70 & 65.20 & 1427 & 67.70 \\

                LaneATT~\cite{tabelini2021keep} & ResNet18 & 47.35 & 75.13 & 51.29 & 91.17 & 72.71 & 65.82 & 68.03 & 49.13 & 87.82 & 63.75 & \textbf{1020} & 68.58 \\

                LaneATT~\cite{tabelini2021keep} & ResNet34 & 49.57 & 76.68 & 54.34  & 92.14 & 75.03 & 66.47 & 78.15 & 49.39 & 88.38 & 67.72 & 1330 & 70.72 \\

                LaneATT~\cite{tabelini2021keep} & ResNet122 & 51.48 & 77.02 & 57.50  & 91.74 & 76.16 & 69.47 & 76.31 & 50.46 & 86.29 & 64.05 & 1264 & 70.81 \\
                
                LaneAF~\cite{abualsaud2021laneaf} & ERFNet & 48.60 & 75.63 & 54.53  & 91.10 & 73.32 & 69.71 & 75.81 & 50.62 & 86.86 & 65.02 & 1844 & 70.90 \\
                
                LaneAF~\cite{abualsaud2021laneaf} & DLA34 & 50.42 & 77.41 & 56.79  & 91.80 & 75.61 & 71.78 & 79.12 & 51.38 & 86.88 & 72.70 & 1360 & 73.03 \\
                
                SGNet~\cite{su2021structure} & ResNet18 & - & 76.12 & -  & 91.42 & 74.05 & 66.89 & 72.17 & 50.16 & 87.13 & 67.02 & 1164 & 70.67 \\
                
                SGNet~\cite{su2021structure} & ResNet34 & - & 77.27 & -  & 92.07 & 75.41 & 67.75 & 74.31 & 50.90 & 87.97 & 69.65 & 1373 & 72.69 \\
                
                FOLOLane~\cite{qu2021focus} & ERFNet & - & 78.80 & - & 92.70 & 77.80 & 75.20 & 79.30 & 52.10 & 89.00 & 69.40 & 1569 & 74.50 \\
                
                CondLane~\cite{liu2021condlanenet} & ResNet18 & 51.84 & 78.14 & 57.42  & 92.87 & 75.79 & 70.72 & 80.01 & 52.39 & 89.37 & 72.40 & 1364 & 73.23 \\

                CondLane\cite{liu2021condlanenet} & ResNet34 & 53.11 & 78.74 & 59.39  & 93.38 & 77.14 & 71.17 & 79.93 & 51.85 & 89.89 & 73.88 & 1387 & 73.92 \\

                CondLane\cite{liu2021condlanenet} & ResNet101 & 54.83 & 79.48 & 61.23  & 93.47 & 77.44 & 70.93 & 80.91 & 54.13 & 90.16 & 75.21 & 1201 & 74.80 \\
                CLRNet\cite{5} & ResNet18 & 55.23 & 79.58 & 62.21   & 93.30 & 78.33 & 73.71 & 79.66 &  53.14 &  90.25 &  71.56 & 1321 & 75.11 \\
                CLRNet\cite{5} & ResNet34 & 55.14 &  79.73 &  62.11  &  93.49 & 78.06 & 74.57 & 79.92 & 54.01 & 90.59 & 72.77 &1216 & 75.02\\
                CLRNet\cite{5} & DLA34 & \textbf{55.64} & \textbf{80.47} & 62.78  & 93.73 & 79.59 & \textbf{75.30} & \textbf{82.51} & \textbf{54.58} & \textbf{90.62} & 74.13 &1155 & 75.37 \\


                \midrule

           
                \textbf{(ours)} & ResNet18 &  55.23 & 79.57 & 62.21   & 93.40 & 78.30 &  73.22 & 80.25 &  52.97 &  90.17 &  71.56 & 1321 & 74.87 \\
                \textbf{(ours)} & DLA34 & 55.50 & 80.10 & \textbf{63.30}  & 93.80 & \textbf{79.90} & 75.10 & 82.33 & 54.40 & 90.49 & \textbf{74.71} &1155 & \textbf{76.02} \\
    
           
                
                \bottomrule
            \end{tabular}
            

        } %

    \end{center}
    \caption{
    %State-of-the-art results on CULane. Since the images in the ``Cross'' category have no lanes, the reported number is the amount of false-positives. For a fairer comparison, we remeasure the FPS of the source code available detectors using one NVIDIA 1080Ti GPU on the same machine, * means FPS on TensorRT. In addition, we rerun the evaluation of these detectors to report the mF1, F1@50, F1@75.
    State-of-the-art results on CULane.  In addition, we also evaluation these detectors to report the mF1, F1@50, F1@75. For ``Cross'' category , only false positives are shown. The reported metric of these categories is based on F1@50.
    }

    \label{tab:culane_main}

\end{table*}



==> tables/overall_ablation.tex <==
\begin{table}[htb]
	\centering
	
	\vspace{0.1cm}
	\addtolength{\tabcolsep}{0pt}
	\resizebox{0.48\textwidth}{!}{%
	\begin{tabular}{*{12}{c}}
		\toprule
		\textbf{Data Preprocessing} & \textbf{Attention Sampling} & \textbf{WE-FPN} & \textbf{Crowded}   & \textbf{Curve}  & \textbf{Night} & \\
		\midrule
		                      &                          &                  &  79.59 & 74.13 & 75.37     \\
		\checkmark            &                          &                  &  79.62 & 74.17 &  75.41    \\
		\checkmark            & \checkmark               &                  &  79.79 & 74.50  & 75.82     \\
		\checkmark            & \checkmark               & \checkmark       & \textbf{79.90} & \textbf{74.71} & \textbf{76.02}   \\
		\bottomrule
	\end{tabular}
	}
	\caption{Effects of each component in our method. Results are reported on CULane.}
	\label{tab:overall-ablation}
	
\end{table}


==> tables/tusimple.tex <==
\begin{table}
    \begin{center}
    \resizebox{0.5\textwidth}{!}{%
            \begin{tabular}{@{}lrrrrrrr@{}}
                \toprule
                \textbf{Method} & \textbf{Backbone}        & \textbf{F1 (\%)} & \textbf{Acc (\%)}  & \textbf{FP (\%)} & \textbf{FN (\%)} \\ \midrule
                
                SCNN~\cite{pan2018spatial} & VGG16 & 95.97 & 96.53  & 6.17 & \textbf{1.80} \\
                
                RESA~\cite{zheng2021resa} & ResNet34 & 96.93 & 96.82 & 3.63 & 2.48  \\
                
                PolyLaneNet~\cite{tabelini2021polylanenet}  & EfficientNetB0 & 90.62 & 93.36 & 9.42 & 9.33 \\
                
                E2E~\cite{yoo2020end}  & ERFNet  & 96.25  & 96.02  & 3.21 & 4.28 \\
                
                UFLD\cite{qin2020ultra} & ResNet18 & 87.87 & 95.82 & 19.05 & 3.92 \\
                
                UFLD\cite{qin2020ultra}  &  ResNet34 & 88.02 & 95.86  & 18.91 & 3.75 \\
                
                LaneATT\cite{tabelini2021keep} & ResNet18 & 96.71 & 95.57 & 3.56 & 3.01 \\
                
                LaneATT\cite{tabelini2021keep} & ResNet34 & 96.77 & 95.63 & 3.53 & 2.92 \\
                
                LaneATT\cite{tabelini2021keep} & ResNet122 & 96.06 & 96.10 & 5.64 & 2.17 \\
                
                FOLOLane\cite{qu2021focus} & ERFNet & 96.59 & \textbf{96.92} & 4.47 & 2.28 \\
                
                CondLaneNet\cite{liu2021condlanenet} & ResNet18 & 97.01 & 95.48 & 2.18 & 3.80 \\
                
                CondLaneNet\cite{liu2021condlanenet} & ResNet34 & 96.98 & 95.37  & 2.20 & 3.82 \\
                \methodname~\cite{5} & ResNet18                                & \textbf{97.89}                                 & 96.84                                 & 2.28                                 & 1.92  \\

                \methodname~\cite{5} &     ResNet34                & 97.82                                 &  96.87                                 & 2.27                                 &  2.08    \\

                \methodname~\cite{5} & ResNet101                               & 97.62                                 &  96.83                                 & 2.37                                 & 2.38    \\ 
                \midrule

                
                \textbf{\methodname~(ours)} & ResNet18                               & 97.70                                 &  96.66                                 & \textbf{2.12}                                 & 2.42    \\ 
                \bottomrule
            \end{tabular}
    }

    \end{center}
    \caption{State-of-the-art results on TuSimple. Additionally, F1 was computed using the official source code.}

    \label{tab:tusimple_main}

\end{table}


% \begin{table}
%     \begin{center}
%     \resizebox{0.5\textwidth}{!}{%
%             \begin{tabular}{@{}lrrrrrrr@{}}
%                 \toprule
%                 \textbf{Method} & \textbf{Backbone}        & \textbf{F1 (\%)} & \textbf{Acc (\%)}  & \textbf{FPS} & \textbf{MACs (G)} & \textbf{FP (\%)} & \textbf{FN (\%)} \\ \midrule
                
%                 SCNN~\cite{pan2018spatial} & VGG16 & 95.97 & 96.53 & 7.5 & - & 6.17 & 1.80 \\
                
%                 RESA~\cite{zheng2021resa} & ResNet34 & 96.93 & 96.82 & - & - & 3.63 & 2.48  \\
                
%                 PolyLaneNet~\cite{tabelini2021polylanenet}  & EfficientNetB0 & 90.62 & 93.36 & 115 & 1.7 & 9.42 & 9.33 \\
                
%                 E2E~\cite{yoo2020end}  & ERFNet  & 96.25  & 96.02  & - & - & 3.21 & 4.28 \\
                
%                 UFLD\cite{qin2020ultra} & ResNet18 & 87.87 & 95.82 & 312.5 & - & 19.05 & 3.92 \\
                
%                 UFLD\cite{qin2020ultra}  &  ResNet34 & 88.02 & 95.86 & 169.5 & - & 18.91 & 3.75 \\
                
%                 LaneATT\cite{tabelini2021keep} & ResNet18 & 96.71 & 95.57 & 250 & 9.3 & 3.56 & 3.01 \\
                
%                 LaneATT\cite{tabelini2021keep} & ResNet34 & 96.77 & 95.63 & 171 & 18.0 & 3.53 & 2.92 \\
                
%                 LaneATT\cite{tabelini2021keep} & ResNet122 & 96.06 & 96.10 & 26 & 70.5 & 5.64 & 2.17 \\
                
%                 FOLOLane\cite{qu2021focus} & ERFNet & 96.59 & 96.92 & - & - & 4.47 & 2.28 \\
                
%                 CondLaneNet\cite{liu2021condlanenet} & ResNet18 & 97.01 & 95.48 & 220 & 10.2 & 2.18 & 3.80 \\
                
%                 CondLaneNet\cite{liu2021condlanenet} & ResNet34 & 96.98 & 95.37 & 154 & 19.6 & 2.20 & 3.82 \\
                
%                 CondLaneNet\cite{liu2021condlanenet} & ResNet101 & 97.24 & 96.54 & 58 & 44.8 & 2.01 & 3.50 \\
%                 \midrule

%                 \textbf{\methodname} & ResNet18                                & 95.57                                 & \underline{3.56}                                 & 3.01                                 & \underline{250}                              & \underline{9.3} \\

%                 \textbf{\methodname}  &     ResNet34                & 95.63                                 & \textbf{3.53}                                 & 2.92                                 & 171                              & 18.0 \\

%                 \textbf{\methodname} & ResNet101                               & 96.10                                 & 5.64                                 & 2.17                                 & 26                               & 70.5 \\ 
%                 \textbf{\methodname}  & ERFNet                                & 96.10                                 & 5.64                                 & 2.17                                 & 26                               & 70.5 \\ \bottomrule
                

%             \end{tabular}
%     }

%     \end{center}
%     \caption{State-of-the-art results on TuSimple. For a fairer comparison, the FPS of the fastest method (\cite{ufsa}) was measured on the same machine and conditions as our method. Additionally, all metrics for this method were computed using the official source code, since only the accuracy was available in the paper.}

%     \label{tab:tusimple_main}

% \end{table}

